Pipe-BD: Pipelined Parallel Blockwise Distillation

Training large deep neural network models is highly challenging due to their tremendous computational and memory requirements. Blockwise distillation provides one promising method towards faster convergence by splitting a large model into multiple smaller models. In state-of-the-art blockwise distillation methods, training is performed block-by-block in a data-parallel manner using multiple GPUs. To produce inputs for the student blocks, the teacher model is executed from the beginning until the current block under training. However, this results in a high overhead of redundant teacher execution, low GPU utilization, and extra data loading. To address these problems, we propose Pipe-BD, a novel parallelization method for blockwise distillation. Pipe-BD aggressively utilizes pipeline parallelism for blockwise distillation, eliminating redundant teacher block execution and increasing per-device batch size for better resource utilization. We also extend to hybrid parallelism for efficient workload balancing. As a result, Pipe-BD achieves significant acceleration without modifying the mathematical formulation of blockwise distillation. We implement Pipe-BD on PyTorch, and experiments reveal that Pipe-BD is effective on multiple scenarios, models, and datasets.

==> alg_js.tex <==

\begin{algorithm}
\caption{\scheme procedure}
\begin{algorithmic}[1]

 \renewcommand{\algorithmicrequire}{\textbf{Input:}}
%  \renewcommand{\algorithmicensure}{\textbf{Output:}}
 \REQUIRE $ $ \\
 \hspace*{\algorithmicindent}$G$: \#devices, $D_i$: $i$th device\\
 \hspace*{\algorithmicindent}$D_{prev/next}$: previous/next device in teacher relaying\\
 \hspace*{\algorithmicindent}$T_i$: $i$th teacher block, $S_i$: $i$th student block
  \vspace{2mm}
%  \ENSURE  out
 \\ \textit{\textbf{Initialization}: load scheduled $T_i$s and $S_i$s to each device}
  \vspace{2mm}
%   \STATE 
%  \\ \textit{LOOP Process}
  \FOR {each $g = 0$ ... $G$}
    \FOR {each step}
    % \STATE {\color{blue(ncs)}{// feature map array for students}}
    % \STATE guide\_fms = []
    % \STATE temp\_fm \textleftarrow \textit{RECV} feature map from $D_{prev}$ %{\color{blue(ncs)}{// TR}}
    \STATE \textit{RECV} teacher feature map from $D_{prev}$ {\color{blue(ncs)}{// TR}}
    % \STATE guide\_fms.push\_back(temp\_fm)
    \FOR {each $T_i$ loaded on $D_g$}
        % \STATE temp\_fm \textleftarrow \textit{FWD} ($T_i$, temp\_fm)
        \STATE \textit{FWD} $T_i$
        % \STATE guide\_fms.push\_back(temp\_fm)
    \ENDFOR
    % \STATE \textit{SEND} temp\_fm to $D_{next}$ %{\color{blue(ncs)}{// TR}}
    \STATE \textit{SEND} last teacher feature map to $D_{next}$ {\color{blue(ncs)}{// TR}}
    \FOR {each $S_i$ loaded on $D_g$}
        % \STATE {\color{blue(ncs)}{// load feature map for student FWD}}
        % \STATE fm \textleftarrow guide\_fms.pop\_front()
        % \STATE {\color{blue(ncs)}{// load teacher output for student BWD}}
        % \STATE teacher\_output \textleftarrow guide\_fms.peek()
        % \STATE \textit{FWD/BWD} ($S_i$, fm, teacher\_output)
        \STATE \textit{FWD/BWD} $S_i$
    \ENDFOR
  \IF {$TYPE ==$ AHD}
  \STATE \textit{ALL\_REDUCE} data-parallel gradient {\color{blue(ncs)}{// AHD}}
  \ENDIF
%   \IF {$TYPE ==$ DPU or AHD}
%   \STATE \textit{UPDATE} in decoupled manner %{\color{blue(ncs)}{// DPU, AHD}}
%   \ELSE
%   \STATE \textit{UPDATE} in coupled manner %{\color{blue(ncs)}{// TR}}
%   \ENDIF
    \IF {$TYPE ==$ DPU or AHD}
    \STATE \textit{UPDATE\_{decoupled}} {\color{blue(ncs)}{// DPU}} \textbf{else} \textit{UPDATE}
    \ENDIF
%   \STATE \textbf{go to} line 3 \textbf{if} step remains.
  \ENDFOR
  \ENDFOR
 \end{algorithmic} 
 \end{algorithm}

==> archive.tex <==


\begin{comment}
\subsection{Algorithm}
To find the best partitioning that satisfies~\cref{sec:reconfg:problem}, \dr builds 2-level tree and grid-searches the best one.
The first-level is decided by data-parallel configuration.
The second-level covers all possible configurations under the first-level data-parallel configuration.
@@ shows the tree for the environment of 4 blocks and 4 GPUs.
The first-level has @@@@ cases, and the second-level contains every cases under dedicated first-level setting.
\Bd generally has @@ blocks, so the size of tree and the searching space are not large.
\JS{I'll draw 2-level search graph here...}


\end{comment}



\subsection{Reconfiguration}
\subsubsection{Problem Formulation}
\label{sec:reconfg:problem}

\begin{figure}
\centering
 \includegraphics[width=\columnwidth]{figs/scheduling_problem.pdf}
 \caption{Problem formulation of \dr.}
 \label{fig:sched_prob}
\end{figure}

\hfill

\textbf{Definition} \emph{Blockwise Pipeline Dependency Graph (BPDG)} reflects the dependency among blocks as depicted in \cref{fig:sched_prob}.
In \bd, each block has a (teacher, student) pair, and it is regarded as node.
This node has two properties; teacher execution time ($T_i$) and student execution time ($S_i$).
The dependency among blocks are represented as an edge between nodes.
An edge has a communication time between blocks ($C_i$) as a attribute.

\textbf{Objective}
%\JL{@JY: could you get a bit more formal? i.e., use equations rather than sentences} \JS{I'll fix this part more formal...}
\Dr is to find the configuration that makes the minimum total pipeline execution time.
We can convert this problem into partitioning of BPDG as illustrated in~\cref{fig:sched_prob}.
Each partition means the working set for specific GPUs.

Given, 
\begin{align}
k &: block_k \in Partition_j \notag \\
g_j &: \#GPUs\;for\;Patition_j\notag\\
DPC_j &: dp\;gradient\;sharing\;time\notag
\end{align}

Then, a partition execution time ($P_j$) and the objective are,
\begin{align}
P_j = sum(T_k+S_k)/g_j + DPC_j \;\notag\\
TotalExecTime \propto max(P_j)\notag\\
\therefore\;\textbf{Objective} : argmin_{config}max(P)
    \label{eq:res}
\end{align}
Note that $C_i$ is omitted in this objective for brevity because it is negligible compared to other execution times due to the fast interconnect and overlapping.





\JL{choose between below two}
\JL{1} we simply assume that the execution time is proportional to the batchsize. 
This model will cause some errors due to the GPU resource utilizations, but such error will be corrected during monitoring during the next epoch and will lead to another reconfiguration next epoch.





In the formulation of \cref{sec:reconfg:problem}, there are three\JL{@@check@@} workload dependent performance variables: $T_i+S_i$ (Average block execution time depending on the batchsize) and $DPC_i$ (Average gradient sharing time).%, and @@ (Average teacher relaying time).
Although the parameters seem to be constant once a workload is decided, those can change during the training.
For neural networks that employ dynamic architecture~\cite{proxyless, dance}, the architecture is chosen probabilistically according to some trained parameters.
As the training goes on, the parameter will change its value and hence the average block execution time will change accordingly.
In addition, increase in the device temperature also contributes to the change in those variables.

To adapt to those changes, each device monitors the performance variables and checks if the monitored values differ from what has been stored.
If the system-wide difference exceeds certain threshold, reconfiguration takes place.
Based on the current observed values, a new optimal schedule is calculated.
Considering the practical problem size of @@, complexity of @@ can be explored using exhaustive search.
For estimating @@ and @@ of different batchsizes that have not been observed, 

==> quality_table.tex <==
\begin{table*}[t]
\centering
\small
\begin{tabular}{llcccc}
\toprule
\textbf{Task} & \textbf{Method} & \textbf{\#Params (M)} & \textbf{FLOPs (M)} & \textbf{Accuracy (\%)} \\ \midrule
\multirow{5}{*}{\textbf{Cifar-10}}
& MobileNet V2 (human) & 2.24 & 87.98 & 95.42 \\ 
& ProxylessNAS & 1.31 & 117.4 & 95.44 \\
& ProxylessNAS (w/ FLOPs) & 1.1 & 37.75 & 93.58 \\
& Ours & 1.4 & 76.1 & 95.48 \\
& Ours (w/ FLOPs) & 1.16 & 65.3 & 95.31 \\\midrule
\multirow{4}{*}{\textbf{ImageNet}}
& ProxylessNAS & 7.1 & 465 & 75.1 \\
& ProxylessNAS (w/ FLOPs) & 4 & 320 & 74.6 \\
& Ours & 4.22 & 420 & @@ \\
& Ours (w/ FLOPs) & 3.86 & 365 & @@ \\\bottomrule
\end{tabular}
\caption{NAS training quality results}
\label{tab:accuracy:nas}
\end{table*}

